A Convolutional Neural Network Neutrino Event Classifier

Convolutional neural networks (CNNs) have been widely applied in the computer vision community to solve complex problems in image recognition and analysis. We describe an application of the CNN technology to the problem of identifying particle interactions in sampling calorimeters used commonly in high energy physics and high energy neutrino physics in particular. Following a discussion of the core concepts of CNNs and recent innovations in CNN architectures related to the field of deep learning, we outline a specific application to the NOvA neutrino detector. This algorithm, CVN (Convolutional Visual Network) identifies neutrino interactions based on their topology without the need for detailed reconstruction and outperforms algorithms currently in use by the NOvA collaboration.

==> Makefile <==
all:
	pdflatex cvn_paper.tex
	pdflatex cvn_paper.tex
	bibtex   cvn_paper
	pdflatex cvn_paper.tex
	pdflatex cvn_paper.tex

#	dvips cvn_paper.dvi -o cvn_paper.ps
#	ps2pdf cvn_paper.ps

clean:
	@ls cvn_paper.* | grep -v '.tex\|.bib' | xargs -I {} rm {}



